Exposure-Aware Recommendation using Contextual Bandits

Exposure bias is a well-known issue in recommender systems where items and suppliers are not equally represented in the recommendation results. This is especially problematic when bias is amplified over time as a few items (e.g., popular ones) are repeatedly over-represented in recommendation lists and users' interactions with those items will amplify bias towards those items over time resulting in a feedback loop. This issue has been extensively studied in the literature on model-based or neighborhood-based recommendation algorithms, but less work has been done on online recommendation models, such as those based on top-K contextual bandits, where recommendation models are dynamically updated with ongoing user feedback. In this paper, we study exposure bias in a class of well-known contextual bandit algorithms known as Linear Cascading Bandits. We analyze these algorithms on their ability to handle exposure bias and provide a fair representation for items in the recommendation results. Our analysis reveals that these algorithms tend to amplify exposure disparity among items over time. In particular, we observe that these algorithms do not properly adapt to the feedback provided by the users and frequently recommend certain items even when those items are not selected by users. To mitigate this bias, we propose an Exposure-Aware (EA) reward model that updates the model parameters based on two factors: 1) user feedback (i.e., clicked or not), and 2) position of the item in the recommendation list. This way, the proposed model controls the utility assigned to items based on their exposure in the recommendation list. Extensive experiments on two real-world datasets using three contextual bandit algorithms show that the proposed reward model reduces exposure bias amplification in long run while maintaining the recommendation accuracy.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tbl2.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\aboverulesep=0ex % Solution part 1 of 3
\belowrulesep=0ex % Solution part 1 of 3
\footnotesize
% \small
\centering
\setlength{\tabcolsep}{3pt}
\captionof{table}{Comparison of original and exposure-aware contextual bandits in terms of exposure fairness for items after $T$ rounds of recommendation operation. The bolded entries show the best values and the underlined entries show the statistically significant change with
$p<0.1$.} \label{res}
\begin{tabular}{ll|rrrr|rrrr}
\midrule
\midrule
 \multirow{2}{*}{algorithms} & \multirow{2}{*}{parameters} & \multicolumn{4}{c|}{Amazon Book} & \multicolumn{4}{c}{MovieLens} \\\cline{3-6}\cline{7-10}
 
 &  & $\#clicks\uparrow$ & $EO\downarrow$ & $EI\downarrow$ & $IC\uparrow$ & $\#clicks\uparrow$ & $EO\downarrow$ & $EI\downarrow$ & $IC\uparrow$ \\
 \midrule

 \algname{CascadeLSB} & $c=0.01$ & & & & & 28,368 & 0.947 & 0.983 & 0.572 \\
 \algname{CascadeLSB} & $c=0.25$ & & & & & 31,925 & 0.979 & 0.991 & 0.191 \\
 \algname{CascadeLSB} & $c=1$ & & & & & 33,642 & 0.988 & 0.995 & 0.567 \\
 \algname{EARSCascadeLSB}  & $c=1,\epsilon=0.05$ &  &  &  &  &  &  &  &  \\
 \algname{EACascadeLSB}  & $c=0.01,\gamma=5e-5,L=1$ & & & & & 27,609 & \textbf{0.939} & \textbf{0.979} & \textbf{0.589} \\
 \algname{EACascadeLSB}  & $c=0.01,\gamma=5e-5,L=5$ &  & & & & 27,760 & \textbf{0.941} & \textbf{0.980} & \textbf{0.602} \\
 \algname{EACascadeLSB} & $c=0.25,\gamma=5e-5,L=1$ & & & & & 30,092 & \underline{\textbf{0.969}} & \underline{\textbf{0.986}} & \textbf{0.263} \\
 \algname{EACascadeLSB} & $c=0.25,\gamma=5e-5,L=5$ & & & & & 29,894 & \underline{\textbf{0.969}} & \underline{\textbf{0.986}} & \textbf{0.279} \\
 \algname{EACascadeLSB} & $c=1,\gamma=5e-5,L=1$ & & & & & 32,341 & \underline{\textbf{0.984}} & \textbf{0.992} & \underline{\textbf{0.591}} \\
 \algname{EACascadeLSB} & $c=1,\gamma=5e-5,L=5$ & & & & & 32,203 & \underline{\textbf{0.983}} & \textbf{0.992} & \underline{\textbf{0.592}} \\
 \hline
 
 \algname{CascadeLinUCB}  & $c=0.01$ & & & & & 15,706 & 0.731 & 0.764 & 0.944 \\
 \algname{CascadeLinUCB} & $c=0.25$ & & & & & 12,840 & 0.866 & 0.879 & 0.919 \\
 \algname{CascadeLinUCB} & $c=1$ & & & & & 9,870 & 0.932 & 0.939 & 0.799 \\
 \algname{EARSCascadeLinUCB} & $c=1,\epsilon=0.05$ & & & & &  &  &  &  \\
 \algname{EACascadeLinUCB}  & $c=0.01,\gamma=5e-5,L=1$ & & & & & 15,970 & \textbf{0.695} & \textbf{0.727} & \textbf{0.953} \\
 \algname{EACascadeLinUCB}  & $c=0.01,\gamma=5e-5,L=5$ & & & & & 15,684 & \textbf{0.705} & \textbf{0.731} & \textbf{0.950} \\
 \algname{EACascadeLinUCB} & $c=0.25,\gamma=5e-5,L=1$ & & & & & 15,646 & \underline{\textbf{0.779}} & \underline{\textbf{0.801}} & \textbf{0.943} \\
 \algname{EACascadeLinUCB} & $c=0.25,\gamma=5e-5,L=5$ & & & & & 14,428 & \underline{\textbf{0.789}} & \underline{\textbf{0.810}} & \textbf{0.944} \\
 \algname{EACascadeLinUCB} & $c=1,\gamma=5e-5,L=1$ & & & & & 12,125 & \underline{\textbf{0.874}} & \textbf{0.885} & \underline{\textbf{0.927}} \\
 \algname{EACascadeLinUCB} & $c=1,\gamma=5e-5,L=5$ & & & & & 11,856 & \underline{\textbf{0.885}} & \textbf{0.894} & \underline{\textbf{0.910}} \\
 \hline
 \algname{CascadeHybrid}  & $c=0.01$ & & & & & 21,896 & 0.872 & 0.926 & 0.699 \\
 \algname{CascadeHybrid} & $c=0.25$ & & & & & 30,785 & 0.953 & 0.990 & 0.673 \\
 \algname{CascadeHybrid} & $c=1$ & & & & & 31,491 & 0.972 & 0.994 & 0.350 \\
 \algname{EARSCascadeHybrid} & $c=1,\epsilon=0.05$ & & & & &  &  &  &  \\
 \algname{EACascadeHybrid}  & $c=0.01,\gamma=5e-5,L=1$ & & & & & 24,298 & \textbf{0.871} & \textbf{0.929} & \textbf{0.927} \\
 \algname{EACascadeHybrid}  & $c=0.01,\gamma=5e-5,L=5$ & & & & & 23,328 & \textbf{0.858} & \textbf{0.917} & \textbf{0.937} \\
 \algname{EACascadeHybrid} & $c=0.25,\gamma=5e-5,L=1$ & & & & & 29,342 & \underline{\textbf{0.954}} & \underline{\textbf{0.984}} & \textbf{0.667} \\
 \algname{EACascadeHybrid} & $c=0.25,\gamma=5e-5,L=5$ & & & & & 29,463 & \underline{\textbf{0.954}} & \underline{\textbf{0.985}} & \textbf{0.717} \\
 \algname{EACascadeHybrid} & $c=1,\gamma=5e-5,L=1$ & & & & & 30,345 & \underline{\textbf{0.974}} & \textbf{0.991} & \underline{\textbf{0.424}} \\
 \algname{EACascadeHybrid} & $c=1,\gamma=5e-5,L=5$ & & & & & 30,429 & \underline{\textbf{0.973}} & \textbf{0.991} & \underline{\textbf{0.447}} \\
 \midrule
\midrule
\end{tabular}
\end{table*}


% \captionsetup[table]{skip=4pt}
% \begin{table}[t]
% \aboverulesep=0ex % Solution part 1 of 3
% \belowrulesep=0ex % Solution part 1 of 3
% % \footnotesize
% \small
% \centering
% \setlength{\tabcolsep}{3pt}
% \captionof{table}{Comparison of original and exposure-aware contextual bandits in terms of exposure fairness for items after $T$ rounds of recommendation operation. The bolded entries show the best values and the underlined entries show the statistically significant change with
% $p<0.1$.} \label{res}
% \begin{tabular}{l|rrr|rrr}
% \midrule
% \midrule
%  \multirow{2}{*}{algorithms} & \multicolumn{3}{c|}{Amazon Book} & \multicolumn{3}{c}{MovieLens} \\\cline{2-4}\cline{5-7}
 
%  & $EO$ & $EI$ & $IC$ & $EO$ & $EI$ & $IC$ \\
%  \midrule

%  \algname{CascadeLSB}  & 0.921 & 0.954 & 30.2\% & 0.951 & 0.991 & 51.1\% \\
%  \algname{CascadeLinUCB} & 0.620 & 0.716 & 91.2\% & 0.723 & 0.821 & 94.8\% \\
%  \algname{CascadeHybrid} & 0.607 & 0.736 & 98.8\% & 0.874 & 0.979 & 83.8\% \\
%  \hline
%  \algname{EACascadeLSB}  &  \textbf{0.917} & \textbf{0.952} & \underline{\textbf{32.7\%}} & \textbf{0.947} & \textbf{0.988} & \textbf{52.1\%} \\
%  \algname{EACascadeLinUCB} & \underline{\textbf{0.591}} & \underline{\textbf{0.675}} & \underline{\textbf{93.1\%}} & \underline{\textbf{0.685}} & \underline{\textbf{0.759}} & \textbf{95.4\%} \\
%  \algname{EACascadeHybrid} & \textbf{0.582} & \underline{\textbf{0.711}} & 98.8\% & \underline{\textbf{0.831}} & \textbf{0.965} & \underline{\textbf{90.7\%}} \\
 
%  \midrule
% \midrule
% \end{tabular}
% \end{table}

==> tbl3.tex <==
\captionsetup[table]{skip=4pt}
\begin{table*}[t]
\aboverulesep=0ex % Solution part 1 of 3
\belowrulesep=0ex % Solution part 1 of 3
\footnotesize
% \small
\centering
%\setlength{\tabcolsep}{3pt}
\captionof{table}{Trade-off between the number of clicks and exposure fairness with varying degree of exploration for contextual bandit algorithms on Amazon Book and MovieLens datasets. Percentage increase or decrease achieved by the proposed exposure-aware algorithms compared to the original algorithms is reported. Positive values for $\Delta^{click}$ and $\Delta^{IC}$, and negative values for $\Delta^{EO}$ and $\Delta^{EI}$ indicate improvement by the proposed exposure-aware algorithms.} \label{trade_off}
\begin{tabular}{l|l|rrrr|rrrr}
\midrule
\midrule
 \multirow{2}{*}{algorithm} & \multirow{2}{*}{hyperparameter} & \multicolumn{4}{c|}{Amazon Book} & \multicolumn{4}{c}{MovieLens}\\
 
 \cline{3-10}
 
 & & $\Delta^{click}$ & $\Delta^{EO}$ & $\Delta^{EI}$ & $\Delta^{IC}$ & $\Delta^{click}$ & $\Delta^{EO}$ & $\Delta^{EI}$ & $\Delta^{IC}$ \\

\midrule

 \multirow{6}{*}{\algname{EACascadeLSB}} 
 & $c=0.0001$ & 0.01 & -0.32 & -0.17 & 8.28 & 0.04 & -0.36 & -0.23 & 1.88 \\
 & $c=0.001$ & 0.43 & -0.29 & -0.15 & 12.58 & -0.02 & -0.35 & -0.27 & -2.74 \\
 & $c=0.01$ & 1.13 & -0.43 & -0.14 & 20.07 & -0.11 & -0.29 & -0.23 & -0.06 \\
 & $c=0.25$ & 0.91 & 0.01 & -0.05 & 18.62 & -0.14 & -0.92 & -0.35 & 7.60 \\
 & $c=0.5$ & 2.39 & 0.25 & 0.18 & 9.85 & -0.05 & -0.86 & -0.30 & 5.41 \\
 & $c=1$ & 5.65 & 0.34 & 0.27 & 10.40 & -0.01 & -0.50 & -0.24 & 6.60 \\
 
 \midrule
 
 \multirow{6}{*}{\algname{EACascadeLinUCB}} 
 & $c=0.0001$ & -0.09 & -4.76 & -6.92 & 0.57 & -0.11 & -4.50 & -6.72 & 0.65 \\
 & $c=0.001$ & 0.01 & -9.76 & -11.56 & 1.02 & -0.07 & -5.93 & -8.13 & 1.75 \\
 & $c=0.01$ & -0.50 & -2.75 & -5.74 & 0.25 & 0.07 & -7.43 & -9.22 & 1.52 \\
 & $c=0.25$ & -0.26 & -9.25 & -10.98 & 4.22 & 0.04 & -7.43 & -9.28 & 0.55 \\
 & $c=0.5$ & 0.77 & -10.82 & -11.53 & 3.68 & 0.21 & -8.28 & -9.14 & 1.41 \\
 & $c=1$ & 2.32 & -13.14 & -11.58 & 5.17 & 0.21 & -9.03 & -8.24 & 2.61 \\
 
 \midrule
 
 \multirow{6}{*}{\algname{EACascadeHybrid}} 
 & $c=0.0001$ & 4.71 & -4.20 & -1.19 & 0.05 &  0.24 & -0.18 & -2.04 & 0.47 \\
 & $c=0.001$ & -1.78 & 5.19 & 7.31 & -2.13 & 0.44 & -2.39 & -1.37 & 3.14 \\
 & $c=0.01$ & 1.18 & -5.05 & -3.77 & 9.22 & 0.13 & 0.40 & -1.78 & 2.20 \\
 & $c=0.25$ & 5.36 & -9.91 & -5.35 & 11.13 & 0.03 & -2.70 & -1.95 & 11.49 \\
 & $c=0.5$ & 4.85 & -10.30 & -5.04 & 24.11 & 0.47 & -4.75 & -1.27 & 0.70 \\
 & $c=1$ & 8.85 & -4.85 & -1.70 & 19.03 & 0.20 & -7.06 & -2.63 & 15.86 \\
 
 \midrule
 \midrule
\end{tabular}
\end{table*}

% \captionsetup[table]{skip=4pt}
% \begin{table*}[t]
% \aboverulesep=0ex % Solution part 1 of 3
% \belowrulesep=0ex % Solution part 1 of 3
% % \footnotesize
% \small
% \centering
% %\setlength{\tabcolsep}{3pt}
% \captionof{table}{Trade-off between the number of clicks and exposure fairness with varying degree of exploration for contextual bandit algorithms on Amazon Book dataset. Percentage increase or decrease achieved by the proposed exposure-aware algorithms compared to the original algorithms is reported. Positive values for $clicks$ and negative values for $EO$ indicate improvement by the proposed exposure-aware algorithms.} \label{res_amazonbook}
% \begin{tabular}{l|rr|rr|rr|rr|rr|rr}
% \midrule
% \midrule
%  \multirow{2}{*}{algorithm} & \multicolumn{2}{r|}{$c=0.0001$} & \multicolumn{2}{r|}{$c=0.001$} & \multicolumn{2}{r|}{$c=0.01$} & \multicolumn{2}{r|}{$c=0.25$} & \multicolumn{2}{c|}{$c=0.5$} & \multicolumn{2}{c}{$c=1$} \\
 
% %  \cline{2-13}
 
%  \cline{2-13}
 
%  & $\Delta^{click}$ & $\Delta^{EO}$ & $\Delta^{click}$ & $\Delta^{EO}$ & $\Delta^{click}$ & $\Delta^{EO}$ & $\Delta^{click}$ & $\Delta^{EO}$ & $\Delta^{click}$ & $\Delta^{EO}$ & $\Delta^{click}$ & $\Delta^{EO}$ \\
%  \midrule

%  \algname{EACascadeLSB} & 0.02 & -0.32 & 0.44 & -0.29 & 1.13 & -0.43 & 0.91 & 0.01 & 2.39 & 0.25 & 5.65 & 0.34 \\
%  \algname{EACascadeLinUCB} & -0.09 & -4.77 & 0.01 & -9.76 & -0.50 & -2.75 & -0.26 & -9.25 & 0.77 & -10.82 & 2.32 & -13.14 \\
%  \algname{EACascadeHybrid} & 4.71 & -4.21 & -1.78 & 5.19 & 1.18 & -5.05 & 5.36 & -9.91 & 4.84 & -10.30 & 8.84 & -4.85 \\
 
%  \midrule
%  \midrule
% \end{tabular}
% \end{table*}






% \captionsetup[table]{skip=4pt}
% \begin{table*}[t]
% \aboverulesep=0ex % Solution part 1 of 3
% \belowrulesep=0ex % Solution part 1 of 3
% %\footnotesize
% \small
% \centering
% %\setlength{\tabcolsep}{3pt}
% \captionof{table}{} \label{res}
% \begin{tabular}{l|rr|rrrrrrrrrr}
% \midrule
% \midrule
%  \multirow{3}{*}{hyperparameter} & \multicolumn{6}{c}{Amazon Book} & \multicolumn{6}{c}{MovieLens} \\
 
%   & \multicolumn{2}{r}{\algname{CascadeLSB}} & \multicolumn{2}{r}{\algname{CascadeLinUCB}} & \multicolumn{2}{r}{\algname{CascadeHybrid}} & \multicolumn{2}{r}{\algname{CascadeLSB}} & \multicolumn{2}{c}{\algname{CascadeLinUCB}} & \multicolumn{2}{c}{\algname{CascadeHybrid}} \\
%  \midrule
%  & click & gini & click & gini & click & gini & click & gini & click & gini & click & gini \\
%  \midrule

%  $c=0.0001$ & &  &  &  &  &  &  &  &  &  &  &  \\
%  $c=0.001$ & &  &  &  &  &  &  &  &  &  &  &  \\
%  $c=0.01$ & &  &  &  &  &  &  &  &  &  &  &  \\
%  $c=0.25$ & &  &  &  &  &  &  &  &  &  &  &  \\
%  $c=0.5$ & &  &  &  &  &  &  &  &  &  &  &  \\
%  $c=1$ & &  &  &  &  &  &  &  &  &  &  &  \\
 
%  \midrule
%  \midrule
% \end{tabular}
% \end{table*}
